Learning from Implicit User Feedback, Emotions and Demographic Information in Task-Oriented and Document-Grounded Dialogues

Implicit user feedback, user emotions and demographic information have shown to be promising sources for improving the accuracy and user engagement of responses generated by dialogue systems. However, the influence of such information on task completion and factual consistency, which are important criteria for task-oriented and document-grounded dialogues, is not yet known. To address this, we introduce FEDI, the first English task-oriented and document-grounded dialogue dataset annotated with this information. Our experiments with Flan-T5, GPT-2 and Llama 2 show a particularly positive impact on task completion and factual consistency. Participants in our human evaluation reported that the responses generated by the feedback-trained models were more informative (Flan-T5 and GPT-2), relevant and factual consistent (Llama 2).

==> tables/dataset/error_types_short.tex <==
\resizebox*{\linewidth}{!}{
\begin{tabular}{ll}
\multicolumn{1}{c}{\textbf{Error Type}}  & \multicolumn{1}{c}{\textbf{Definition}}                                                                     \\ \hline
\multicolumn{1}{l|}{Ignore Question}     & The system utterance ignores the user's question.                                                           \\ \hline
\multicolumn{1}{l|}{Ignore Request}      & \begin{tabular}[c]{@{}l@{}}The system utterance ignores the user's request to \\ do something.\end{tabular} \\ \hline
\multicolumn{1}{l|}{Ignore Expectation}  & \begin{tabular}[c]{@{}l@{}}The system utterance does not fulfill the user's \\ expecation.\end{tabular}     \\ \hline
\multicolumn{1}{l|}{Attribute Error} &
  \begin{tabular}[c]{@{}l@{}}The system utterance suggests that it did not get \\ the attributes/slots right.\end{tabular} \\ \hline
\multicolumn{1}{l|}{Factually Incorrect} & \begin{tabular}[c]{@{}l@{}}The system utterance contains factually incorrect \\ information.\end{tabular}   \\ \hline
\multicolumn{1}{l|}{Topic Transition Error} &
  \begin{tabular}[c]{@{}l@{}}The system utterance transitions to another / a \\ previous topic without reasonable explanations.\end{tabular} \\ \hline
\multicolumn{1}{l|}{Conversationality}   & \begin{tabular}[c]{@{}l@{}}The system utterance indicates that the system \\ lost track.\end{tabular}       \\ \hline
\multicolumn{1}{l|}{Unclear Intention} &
  \begin{tabular}[c]{@{}l@{}}The system utterance suggests that the user's \\ intent was not successfully conveyed.\end{tabular} \\ \hline
\multicolumn{1}{l|}{Lack of Sociality} &
  \begin{tabular}[c]{@{}l@{}}The system utterance lacks consideration of \\ social standards, is toxic or disrespectful.\end{tabular}
\end{tabular}}

==> tables/dataset_stats/dataset_and_split_sizes_scenario_based.tex <==
\resizebox*{\linewidth}{!}{
\begin{tabular}{lrrrrrrrrrrr}
 &
  \multicolumn{2}{c}{\textbf{Non-Erroneous}} &
  \multicolumn{8}{c}{\textbf{Erroneous}} &
  \multicolumn{1}{l}{} \\ \hline
 &
  \multicolumn{2}{c}{\textbf{}} &
  \multicolumn{2}{c}{\textbf{Original}} &
  \multicolumn{2}{c}{\textbf{Stage 1}} &
  \multicolumn{2}{c}{\textbf{Stage 2}} &
  \multicolumn{2}{c}{\textbf{Stage 3}} &
  \multicolumn{1}{l}{} \\ \hline
 &
  \multicolumn{1}{l}{\textbf{Train}} &
  \multicolumn{1}{l|}{\textbf{Dev}} &
  \multicolumn{1}{l}{\textbf{Train}} &
  \multicolumn{1}{l|}{\textbf{Dev}} &
  \multicolumn{1}{l}{\textbf{Train}} &
  \multicolumn{1}{l|}{\textbf{Dev}} &
  \multicolumn{1}{l}{\textbf{Train}} &
  \multicolumn{1}{l|}{\textbf{Dev}} &
  \multicolumn{1}{l}{\textbf{Train}} &
  \multicolumn{1}{l|}{\textbf{Dev}} &
  \multicolumn{1}{l}{\textbf{Test}} \\ \hline
\multicolumn{1}{l|}{\textbf{Post Office Task}} &
  373 &
  \multicolumn{1}{r|}{40} &
  386 &
  \multicolumn{1}{r|}{42} &
  386 &
  \multicolumn{1}{r|}{42} &
  386 &
  \multicolumn{1}{r|}{42} &
  386 &
  \multicolumn{1}{r|}{42} &
  77 \\ \hline
\multicolumn{1}{l|}{\textbf{Receptionist Task}} &
  183 &
  \multicolumn{1}{r|}{20} &
  215 &
  \multicolumn{1}{r|}{23} &
  215 &
  \multicolumn{1}{r|}{23} &
  215 &
  \multicolumn{1}{r|}{23} &
  215 &
  \multicolumn{1}{r|}{23} &
  42 \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Question Answering\\ in the Financial and\\ Insurance Domain\end{tabular}}} &
  943 &
  \multicolumn{1}{r|}{103} &
  945 &
  \multicolumn{1}{r|}{105} &
  945 &
  \multicolumn{1}{r|}{105} &
  945 &
  \multicolumn{1}{r|}{105} &
  945 &
  \multicolumn{1}{r|}{105} &
  207 \\ \hhline{============}
\multicolumn{1}{l|}{\textbf{Per Split}} &
  1,499 &
  \multicolumn{1}{r|}{163} &
  1,546 &
  \multicolumn{1}{r|}{170} &
  1,546 &
  \multicolumn{1}{r|}{170} &
  1,546 &
  \multicolumn{1}{r|}{170} &
  1,546 &
  \multicolumn{1}{r|}{170} &
  326 \\ \hline
\multicolumn{1}{l|}{\textbf{Total}} &
  \multicolumn{11}{r}{8,852}
\end{tabular}}

==> tables/dataset_stats/intent_accuracies.tex <==
\resizebox*{\linewidth}{!}{
\begin{tabular}{lrrrrrr}
 &
  \multicolumn{1}{l}{\textbf{Non-Erroneous}} &
  \multicolumn{4}{l}{\textbf{Erroneous}} &
  \multicolumn{1}{l}{\textbf{Test}} \\ \hline
 &
  \multicolumn{1}{l}{\textbf{}} &
  \multicolumn{1}{l}{\textbf{Original}} &
  \multicolumn{1}{l}{\textbf{Stage 1}} &
  \multicolumn{1}{l}{\textbf{Stage 2}} &
  \multicolumn{1}{l}{\textbf{Stage 3}} &
  \multicolumn{1}{l}{\textbf{}} \\ \hline
\multicolumn{1}{l|}{\textbf{Post Office Task}} &
  \multicolumn{1}{r|}{90.21\%} &
  \multicolumn{1}{r|}{81.99\%} &
  \multicolumn{1}{r|}{81.99\%} &
  \multicolumn{1}{r|}{81.99\%} &
  \multicolumn{1}{r|}{81.99\%} &
  73.21\% \\ \hline
\multicolumn{1}{l|}{\textbf{Receptionist Task}} &
  \multicolumn{1}{r|}{97.81\%} &
  \multicolumn{1}{r|}{99.16\%} &
  \multicolumn{1}{r|}{99.16\%} &
  \multicolumn{1}{r|}{99.16\%} &
  \multicolumn{1}{r|}{99.16\%} &
  88.89\% \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Question Answering\\ in the Financial and\\ Insurance Domain\end{tabular}}} &
  \multicolumn{1}{r|}{98.94\%} &
  \multicolumn{1}{r|}{61.13\%} &
  \multicolumn{1}{r|}{99.9\%} &
  \multicolumn{1}{r|}{99.81\%} &
  \multicolumn{1}{r|}{99.71\%} &
  90.39\%
\end{tabular}}

==> tables/dataset_stats/lexical_diversity_comparison.tex <==
\resizebox*{\linewidth}{!}{
\begin{tabular}{lcrrrr}
 &
  \textbf{Type} &
  \multicolumn{1}{c}{\textbf{\#Dialog}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}\#Turns \\ (Avg.)\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Utt. Length\\ (Avg.)\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Lexical\\ Diversity\end{tabular}}} \\ \hline
\multicolumn{1}{l|}{\textbf{MultiWoZ}}     & \multicolumn{1}{c|}{HH} & \multicolumn{1}{r|}{8,5k}    & \multicolumn{1}{r|}{13.7}     & \multicolumn{1}{r|}{6.6}     & 66.23 \\ \hline
\multicolumn{1}{l|}{\textbf{SGD}}                & \multicolumn{1}{c|}{HH} & \multicolumn{1}{r|}{1,6k}    & \multicolumn{1}{r|}{14.5}     & \multicolumn{1}{r|}{4.3}     & 65.0  \\ \hline
\multicolumn{1}{l|}{\textbf{EmpatheticDialogue}} & \multicolumn{1}{c|}{HH}   & \multicolumn{1}{r|}{25k} & \multicolumn{1}{r|}{4.3}  & \multicolumn{1}{r|}{13.7} & 64.2  \\ \hline
\multicolumn{1}{l|}{\textbf{PersonaChat}}        & \multicolumn{1}{c|}{HH} & \multicolumn{1}{r|}{11k} & \multicolumn{1}{r|}{14.8} & \multicolumn{1}{r|}{14.2} & 43.6  \\ \hline
\multicolumn{1}{l|}{\textbf{SaferDialogues}}     & \multicolumn{1}{c|}{HB} & \multicolumn{1}{r|}{}    & \multicolumn{1}{r|}{}     & \multicolumn{1}{r|}{}     & 77.46 \\ \hline
\multicolumn{1}{l|}{\textbf{FITS}}               & \multicolumn{1}{c|}{HB} & \multicolumn{1}{r|}{}    & \multicolumn{1}{r|}{}     & \multicolumn{1}{r|}{}     & 52.78 \\ \hline
\multicolumn{1}{l|}{\textbf{PersonaChatGen}}     & \multicolumn{1}{c|}{A}  & \multicolumn{1}{r|}{1,6k}    & \multicolumn{1}{r|}{16.0}     & \multicolumn{1}{r|}{9.5}     & 56.67 \\ \hline
\multicolumn{1}{l|}{\textbf{SODA}}               & \multicolumn{1}{c|}{A}  & \multicolumn{1}{r|}{1,5M}    & \multicolumn{1}{r|}{7.6}     & \multicolumn{1}{r|}{16.1}     & 68.0  \\ \hhline{======}
\multicolumn{1}{l|}{\textbf{\ourdata}}             & \multicolumn{1}{c|}{A}  & \multicolumn{1}{r|}{8,8k}    & \multicolumn{1}{r|}{7.6}     & \multicolumn{1}{r|}{16.76}     & 62.13
\end{tabular}}

==> tables/dataset_stats/slot_accuracies.tex <==
\resizebox*{\linewidth}{!}{
\begin{tabular}{lrrrrrr}
 &
  \multicolumn{1}{l}{\textbf{Non-Erroneous}} &
  \multicolumn{4}{l}{\textbf{Erroneous}} &
  \multicolumn{1}{l}{\textbf{Test}} \\ \hline
 &
  \multicolumn{1}{l}{\textbf{}} &
  \multicolumn{1}{l}{\textbf{Original}} &
  \multicolumn{1}{l}{\textbf{Stage 1}} &
  \multicolumn{1}{l}{\textbf{Stage 2}} &
  \multicolumn{1}{l}{\textbf{Stage 3}} &
  \multicolumn{1}{l}{\textbf{}} \\ \hline
\multicolumn{1}{l|}{\textbf{Post Office Task}} &
  \multicolumn{1}{r|}{84.02\%} &
  \multicolumn{1}{r|}{65.16\%} &
  \multicolumn{1}{r|}{62.92\%} &
  \multicolumn{1}{r|}{58.73\%} &
  \multicolumn{1}{r|}{57.14\%} &
  29.15\% \\ \hline
\multicolumn{1}{l|}{\textbf{Receptionist Task}} &
  \multicolumn{1}{r|}{74.87\%} &
  \multicolumn{1}{r|}{64.85\%} &
  \multicolumn{1}{r|}{68.31\%} &
  \multicolumn{1}{r|}{69.39\%} &
  \multicolumn{1}{r|}{68.49\%} &
  46.67\% \\ \hline
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Question Answering\\ in the Financial and\\ Insurance Domain\end{tabular}}} &
  \multicolumn{1}{r|}{99.56\%} &
  \multicolumn{1}{r|}{85.29\%} &
  \multicolumn{1}{r|}{99.99\%} &
  \multicolumn{1}{r|}{99.99\%} &
  \multicolumn{1}{r|}{99.99\%} &
  83.85\%
\end{tabular}}

==> tables/experiments/automatic_evaluation.tex <==
\resizebox*{\linewidth}{!}{\begin{tabular}{llrrrrrrrrr}
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Experiment}} & \multicolumn{3}{c}{\textbf{Matching}} & \multicolumn{4}{c}{\textbf{Task Completion}} & \multicolumn{2}{c}{\textbf{Quality}} \\ \hline
 & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{BertScore}} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c}{\textbf{Success}} & \multicolumn{1}{c}{\textbf{Intent Acc.}} & \multicolumn{1}{c|}{\textbf{Slot Acc.}} & \textbf{Toxicity} & \textbf{Q²} \\ \hhline{===========}
\multicolumn{1}{l|}{\multirow{4}{*}{FLAN-T5}} & \multicolumn{1}{l|}{Baseline} & 45.0 & 20.0 & \multicolumn{1}{r|}{88.3} & 86.7 & 85.9 & 54.8 & \multicolumn{1}{r|}{60.9} & 0.02 & 52.7\\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\quad+Demographics} & 43.2 (\textcolor{negative_color}{--1.8}) & 18.4 (\textcolor{negative_color}{--1.6}) & \multicolumn{1}{r|}{87.7 (\textcolor{negative_color}{--0.6})} & 87.0 (\textcolor{positive_color}{+0.3}) & 86.0 (\textcolor{positive_color}{+0.1}) & 33.5 (\textcolor{negative_color}{--21.3}) & \multicolumn{1}{r|}{29.3 (\textcolor{negative_color}{--31.6})} & 0.03 (\textcolor{negative_color}{--0.01})& 54.5 (\textcolor{positive_color}{+1.8}) \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\textbf{\quad+Emotions}} & \textbf{46.7 (\textcolor{positive_color}{+1.7})} & \textbf{21.0 (\textcolor{positive_color}{+1.0})} & \multicolumn{1}{r|}{\textbf{88.9 (\textcolor{positive_color}{+0.6})}} & \textbf{83.9 (\textcolor{negative_color}{--2.8})} & \textbf{83.2 (\textcolor{negative_color}{--2.7})} & \textbf{61.2 (\textcolor{positive_color}{+6.4})} & \multicolumn{1}{r|}{\textbf{58.3 (\textcolor{negative_color}{--2.6})}} & \textbf{0.02} & \textbf{57.5 (\textcolor{positive_color}{+4.8}}) \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\quad+Demographics\\ \quad+Emotions\end{tabular}} & 44.2 (\textcolor{negative_color}{--0.8}) & 19.1 (\textcolor{negative_color}{--0.9}) & \multicolumn{1}{r|}{88.1 (\textcolor{negative_color}{--0.2})} & 85.3 (\textcolor{negative_color}{--1.4}) & 85.1 (\textcolor{negative_color}{--0.8}) & 43.9 (\textcolor{negative_color}{--10.9}) & \multicolumn{1}{r|}{36.7 (\textcolor{negative_color}{--24.2})} & 0.02 & 56.4 (\textcolor{positive_color}{+3.7}) \\ \hhline{===========}
\multicolumn{1}{l|}{\multirow{4}{*}{GPT-2}} & \multicolumn{1}{l|}{Baseline} & 34.9 & 10.4 & \multicolumn{1}{r|}{87.1} & 88.3 & 81.6 & 78.7 & \multicolumn{1}{r|}{69.6} & 0.02 & 28.1 \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\quad+Demographics} & 34.6 (\textcolor{negative_color}{--0.3}) & 10.4 & \multicolumn{1}{r|}{87.1} & 80.2 (\textcolor{negative_color}{--0.1}) & 80.2 (\textcolor{negative_color}{--1.4}) & 69.3 (\textcolor{negative_color}{--9.4}) & \multicolumn{1}{r|}{57.5 (\textcolor{negative_color}{--12.1})} & 0.02 & 26.3 (\textcolor{negative_color}{--1.8}) \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\textbf{\quad+Emotions}} & \textbf{35.1 (\textcolor{positive_color}{+0.2})} & \textbf{10.4} & \multicolumn{1}{r|}{\textbf{87.1}} & \textbf{84.1 (\textcolor{negative_color}{--4.2})} & \textbf{83.8 (\textcolor{positive_color}{+2.2})} & \textbf{75.4 (\textcolor{negative_color}{--3.3})} & \multicolumn{1}{r|}{\textbf{67.3 (\textcolor{negative_color}{--2.3})}} & \textbf{0.02} & \textbf{26.7 (\textcolor{negative_color}{--1.4})} \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\quad+Demographics\\ \quad+Emotions\end{tabular}} & 36.0 (\textcolor{positive_color}{+1.1}) & 11.4 (\textcolor{positive_color}{+1.0}) & \multicolumn{1}{r|}{87.3 (\textcolor{positive_color}{+0.2})} & 85.1 (\textcolor{negative_color}{--3.2}) & 84.8 (\textcolor{positive_color}{+3.2}) & 71.6 (\textcolor{negative_color}{--7.1}) & \multicolumn{1}{r|}{66.7 (\textcolor{negative_color}{-- 2.9})} & 0.02 & 29.2 (\textcolor{positive_color}{+1.1}) \\ \hhline{===========}
\multicolumn{1}{l|}{\multirow{4}{*}{LLaMA}} & \multicolumn{1}{l|}{Baseline} & 30.8 & 8.4 & \multicolumn{1}{r|}{85.7} & 88.3 & 87.3 & 68.7 & \multicolumn{1}{r|}{53.2} & 0.02 & 28.3 \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\quad+Demographics} & 32.9 (\textcolor{positive_color}{+2.1}) & 9.1 (\textcolor{positive_color}{+0.7}) & \multicolumn{1}{r|}{86.3 (\textcolor{positive_color}{+0.6})} & 88.4 (\textcolor{positive_color}{+0.1}) & 88.0 (\textcolor{positive_color}{+0.7}) & 70.9 (\textcolor{positive_color}{+2.2}) & \multicolumn{1}{r|}{54.4 (\textcolor{positive_color}{+1.2})} & 0.02 & 29.0 (\textcolor{positive_color}{+0.7}) \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\textbf{\quad+Emotions}} & \textbf{34.1 (\textcolor{positive_color}{+3.3})} & \textbf{11.5 (\textcolor{positive_color}{+3.1})} & \multicolumn{1}{r|}{\textbf{87.0 (\textcolor{positive_color}{+1.3}})} & \textbf{91.5 (\textcolor{positive_color}{+3.2})} & \textbf{89.9 (\textcolor{positive_color}{+2.6})} & \textbf{68.5 (\textcolor{negative_color}{--0.2})} & \multicolumn{1}{r|}{\textbf{54.7 (\textcolor{positive_color}{+1.5})}} & \textbf{0.02} & \textbf{28.7 (\textcolor{positive_color}{+0.4})} \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\quad+Demographics\\ \quad+Emotions\end{tabular}} & 33.5 (\textcolor{positive_color}{+1.7}) & 10.7 (\textcolor{positive_color}{+2.3}) & \multicolumn{1}{r|}{86.2 (\textcolor{positive_color}{+0.5})} & 91.7 (\textcolor{positive_color}{+3.4}) & 90.0 (\textcolor{positive_color}{+2.7}) & 66.1 (\textcolor{negative_color}{--2.6}) & \multicolumn{1}{r|}{53.6 (\textcolor{positive_color}{+0.4})} & 0.02 & 29.3 (\textcolor{positive_color}{+1.0}) \\ \hhline{===========}
\multicolumn{1}{l|}{\multirow{4}{*}{LLaMA-2}} & \multicolumn{1}{l|}{Baseline} & 29.3 & 7.1 & \multicolumn{1}{r|}{86.1} & 85.9  & 81.2 & 37.6 & \multicolumn{1}{r|}{39.2} & 0.02 & 28.3 \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\quad+Demographics} & 33.8 (\textcolor{positive_color}{+4.5})& 4.5 (\textcolor{negative_color}{--2.6}) & \multicolumn{1}{r|}{86.5 (\textcolor{positive_color}{+0.4})} & 85.6 (\textcolor{negative_color}{--0.3}) & 82.5 (\textcolor{positive_color}{+1.3})& 37.1 (\textcolor{negative_color}{--0.5})& \multicolumn{1}{r|}{40.1 (\textcolor{positive_color}{+0.9})} & 0.02 & 21.3 (\textcolor{negative_color}{--7.0}) \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\textbf{\quad+Emotions}} & \textbf{36.3 (\textcolor{positive_color}{+7.0})} & \textbf{14.9 (\textcolor{positive_color}{+7.8})} &  \multicolumn{1}{r|}{\textbf{85.4 (\textcolor{negative_color}{--0.7})}} & \textbf{89.3 (\textcolor{positive_color}{+3.4})} & \textbf{85.3 (\textcolor{positive_color}{+0.8})} & \textbf{40.2 (\textcolor{positive_color}{+2.6})} & \multicolumn{1}{r|}{\textbf{41.3 (\textcolor{positive_color}{+2.1})}} & \textbf{0.01 (\textcolor{positive_color}{+0.01})} & \textbf{18.7 (\textcolor{negative_color}{--9.6})} \\ \cline{2-11}
\multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\quad+Demographics\\ \quad+Emotions\end{tabular}} & 28.8 (\textcolor{negative_color}{--0.5})& 5.6 (\textcolor{negative_color}{--1.5})& \multicolumn{1}{r|}{81.3 (\textcolor{negative_color}{--4.8})} & 86.7 (\textcolor{positive_color}{+1.8}) & 87.9 (\textcolor{positive_color}{+6.7}) & 41.4 (\textcolor{positive_color}{+3.8}) & \multicolumn{1}{r|}{39.6 (\textcolor{positive_color}{+0.4})} & 0.03 & 20.6 (\textcolor{negative_color}{--7.7})
\end{tabular}}

==> tables/experiments/automatic_evaluation_arxiv.tex <==
\resizebox*{0.7\linewidth}{!}{\begin{tabular}{lrrrr}
\multicolumn{1}{c}{\textbf{Experiment}} & \multicolumn{1}{c}{\textbf{PPL}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{Toxicity}} \\ \hhline{=====}
\multicolumn{1}{l|}{FLAN-T5} & 5.27 & 0.43 & 0.20 & 0.02 \\ \hline
\multicolumn{1}{l|}{\quad+NV} & 5.29 & 0.46 & 0.22 & 0.03 \\ \hline
\multicolumn{1}{l|}{\quad\textbf{+P}} & \textbf{5.47} & \textbf{0.47} & \textbf{0.23} & \textbf{0.02} \\ \hline
\multicolumn{1}{l|}{\quad+NV +P} & 5.41 & 0.46 & 0.22 & 0.03 \\ \hhline{=====}
\multicolumn{1}{l|}{GPT-2} & 4.22 & 0.32 & 0.09 & 0.07 \\ \hline
\multicolumn{1}{l|}{\quad+NV} & 3.83 & 0.32 & 0.09 & 0.07 \\ \hline
\multicolumn{1}{l|}{\quad+P} & 3.61 & 0.32 & 0.09 & 0.09 \\ \hline
\multicolumn{1}{l|}{\quad\textbf{+NV +P}} & \textbf{3.48} & \textbf{0.33} & \textbf{0.10} & \textbf{0.08} \\ \hhline{=====}
\multicolumn{1}{l|}{LLAMA} & 2.65 & 0.32 & 0.10 & 0.04 \\ \hline
\multicolumn{1}{l|}{\quad\textbf{+NV}} & \textbf{2.59} & \textbf{0.31} & \textbf{0.10} & \textbf{0.03} \\ \hline
\multicolumn{1}{l|}{\quad+P} & 2.72 & 0.31 & 0.09 & 0.02 \\ \hline
\multicolumn{1}{l|}{\quad+NV +P} & 2.69 & 0.30 & 0.09 & 0.03
\end{tabular}}

==> tables/experiments/automatic_evaluation_dev.tex <==
\resizebox*{0.9\linewidth}{!}{\begin{tabular}{lrrrrrr}
\multicolumn{1}{c}{\textbf{Experiment}} & \multicolumn{2}{c}{\textbf{Performance}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{2}{c}{\textbf{Task Completion}} \\ \hline
\multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{PPL}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{Toxicity}} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c}{\textbf{Success}} \\ \hhline{=======}
\multicolumn{1}{l|}{\textbf{Flan-T5}} & \textbf{2.01} & \multicolumn{1}{r|}{\textbf{0.42}} & \textbf{0.16} & \multicolumn{1}{r|}{\textbf{0.02}} & \textbf{0.98} & \textbf{0.83} \\ \hline
\multicolumn{1}{l|}{\quad+ NV} & 2.01 & \multicolumn{1}{r|}{0.43} & 0.15 & \multicolumn{1}{r|}{0.03} & 0.98 & 0.83 \\ \hline
\multicolumn{1}{l|}{\quad+ P} & 2.01 & \multicolumn{1}{r|}{0.42} & 0.16 & \multicolumn{1}{r|}{0.03} & 0.98 & 0.83 \\ \hline
\multicolumn{1}{l|}{\quad+ NVP} & 2.03 & \multicolumn{1}{r|}{0.42} & 0.15 & \multicolumn{1}{r|}{0.04} & 0.98 & 0.82 \\ \hhline{=======}
\multicolumn{1}{l|}{GPT-2} & 3.98 & \multicolumn{1}{r|}{0.52} & 0.30 & \multicolumn{1}{r|}{0.07} & 0.99 & 0.92 \\ \hline
\multicolumn{1}{l|}{\quad+ NV} & 3.54 & \multicolumn{1}{r|}{0.55} & 0.30 & \multicolumn{1}{r|}{0.08} & 0.99 & 0.92 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ P}} & \textbf{2.86} & \multicolumn{1}{r|}{\textbf{0.57}} & \textbf{0.32} & \multicolumn{1}{r|}{\textbf{0.09}} & \textbf{0.99} & \textbf{0.91} \\ \hline
\multicolumn{1}{l|}{\quad+ NVP} & 2.98 & \multicolumn{1}{r|}{0.54} & 0.28 & \multicolumn{1}{r|}{0.07} & 0.98 & 0.93 \\ \hhline{=======}
\multicolumn{1}{l|}{LLAMA} & 2.62 & \multicolumn{1}{r|}{0.30} & 0.09 & \multicolumn{1}{r|}{0.05} & 0.73 & 0.60 \\ \hline
\multicolumn{1}{l|}{\quad+ NV} & 2.59 & \multicolumn{1}{r|}{0.31} & 0.10 & \multicolumn{1}{r|}{0.03} & 0.76 & 0.64 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ P}} & \textbf{2.67} & \multicolumn{1}{r|}{\textbf{0.31}} & \textbf{0.09} & \multicolumn{1}{r|}{\textbf{0.02}} & \textbf{0.79} & \textbf{0.62} \\ \hline
\multicolumn{1}{l|}{\quad+ NVP} & 2.63 & \multicolumn{1}{r|}{0.30} & 0.09 & \multicolumn{1}{r|}{0.02} & 0.73 & 0.60 
\end{tabular}}

==> tables/experiments/continuous_learning.tex <==
\resizebox*{0.9\linewidth}{!}{\begin{tabular}{lrrrrrr}
\multicolumn{1}{c}{\textbf{Experiment}} & \multicolumn{3}{c}{\textbf{Performance}} & \multicolumn{1}{c}{\textbf{Quality}} & \multicolumn{2}{c}{\textbf{Task Completion}} \\ \hline
\multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{PPL}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{Toxicity}} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c}{\textbf{Success}} \\ \hhline{=======}
\multicolumn{1}{l|}{FLAN-T5-P} & 4.13 & 0.44 & \multicolumn{1}{r|}{0.20} & \multicolumn{1}{r|}{0.03} & 0.78 & 0.78 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 3.44 & 0.44 & \multicolumn{1}{r|}{0.22} & \multicolumn{1}{r|}{0.03} & 0.77 & 0.78 \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 4.02 & 0.44 & \multicolumn{1}{r|}{0.22} & \multicolumn{1}{r|}{0.03} & 0.76 & 0.82 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ EF}} & \textbf{3.51} & \textbf{0.45} & \multicolumn{1}{r|}{\textbf{0.23}} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.75} & \textbf{0.83} \\ \hhline{=======}
\multicolumn{1}{l|}{GPT-2-PNV} & 3.19 & 0.31 & \multicolumn{1}{r|}{0.11} & \multicolumn{1}{r|}{0.08} & 0.74 & 0.73 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ E}} & \textbf{3.13} & \textbf{0.25} & \multicolumn{1}{r|}{\textbf{0.10}} & \multicolumn{1}{r|}{\textbf{0.07}} & \textbf{0.83} & \textbf{0.80} \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 2.98 & 0.25 & \multicolumn{1}{r|}{0.10} & \multicolumn{1}{r|}{0.09} & 0.82 & 0.80 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.25 & 0.24 & \multicolumn{1}{r|}{0.09} & \multicolumn{1}{r|}{0.09} & 0.84 & 0.81 \\ \hhline{=======}
\multicolumn{1}{l|}{LLAMA-NV} & 3.22 & 0.27 & \multicolumn{1}{r|}{0.06} & \multicolumn{1}{r|}{0.03} & 0.80 & 0.66 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 3.45 & 0.23 & \multicolumn{1}{r|}{0.05} & \multicolumn{1}{r|}{0.03} & 0.73 & 0.62 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ F}} & \textbf{3.23} & \textbf{0.27} & \multicolumn{1}{r|}{\textbf{0.06}} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.81} & \textbf{0.70} \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.28 & 0.25 & \multicolumn{1}{r|}{0.05} & \multicolumn{1}{r|}{0.03} & 0.72 & 0.62
\end{tabular}}

==> tables/experiments/continuous_learning_dev.tex <==
\resizebox*{0.9\linewidth}{!}{\begin{tabular}{lrrrrrr}
\multicolumn{1}{c}{\textbf{}} & \multicolumn{2}{c}{\textbf{Performance}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{2}{c}{\textbf{Task Completion}} \\ \hline
\multicolumn{1}{c|}{\textbf{Experiment}} & \multicolumn{1}{c}{\textbf{PPL}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{Toxicity}} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c}{\textbf{Success}} \\ \hhline{=======}
\multicolumn{7}{c}{\textbf{Stage 1 (Validation)}} \\ \hline
\multicolumn{1}{l|}{Flan-T5-P} & 2.22 & \multicolumn{1}{r|}{0.44} & 0.16 & \multicolumn{1}{r|}{0.03} & 0.94 & 0.61 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 4.04 & \multicolumn{1}{r|}{0.44} & 0.16 & \multicolumn{1}{r|}{0.04} & 0.89 & 0.61 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ F}} & \textbf{2.09} & \multicolumn{1}{r|}{\textbf{0.44}} & \textbf{0.16} & \multicolumn{1}{r|}{\textbf{0.02}} & \textbf{0.89} & \textbf{0.61} \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 1.80 & \multicolumn{1}{r|}{0.44} & 0.16 & \multicolumn{1}{r|}{0.03} & 0.83 & 0.59 \\ \hline
\multicolumn{1}{l|}{\textbf{GPT-2-PNV}} & \textbf{2.09} & \multicolumn{1}{r|}{\textbf{0.43}} & \textbf{0.18} & \multicolumn{1}{r|}{\textbf{0.09}} & \textbf{0.97} & \textbf{0.86} \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 2.16 & \multicolumn{1}{r|}{0.37} & 0.15 & \multicolumn{1}{r|}{0.08} & 0.99 & 0.91 \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 2.20 & \multicolumn{1}{r|}{0.36} & 0.15 & \multicolumn{1}{r|}{0.09} & 0.99 & 0.88 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 1.99 & \multicolumn{1}{r|}{0.32} & 0.13 & \multicolumn{1}{r|}{0.09} & 0.99 & 0.88 \\ \hline
\multicolumn{1}{l|}{\textbf{LLAMA-NV}} & \textbf{3.12} & \multicolumn{1}{r|}{\textbf{0.29}} & \textbf{0.05} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.83} & \textbf{0.66} \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 3.31 & \multicolumn{1}{r|}{0.27} & 0.05 & \multicolumn{1}{r|}{0.03} & 0.87 & 0.66 \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 3.27 & \multicolumn{1}{r|}{0.27} & 0.05 & \multicolumn{1}{r|}{0.04} & 0.78 & 0.57 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.33 & \multicolumn{1}{r|}{0.27} & 0.04 & \multicolumn{1}{r|}{0.03} & 0.82 & 0.60 \\ \hhline{=======}
\multicolumn{7}{c}{\textbf{Stage 2 (Validation)}} \\ \hline
\multicolumn{1}{l|}{Flan-T5-P} & 2.13 & \multicolumn{1}{r|}{0.41} & 0.14 & \multicolumn{1}{r|}{0.03} & 0.82 & 0.73 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ E}} & \textbf{2.15} & \multicolumn{1}{r|}{\textbf{0.44}} & \textbf{0.16} & \multicolumn{1}{r|}{\textbf{0.04}} & \textbf{0.89} & \textbf{0.61} \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 2.22 & \multicolumn{1}{r|}{0.42} & 0.15 & \multicolumn{1}{r|}{0.03} & 0.85 & 0.74 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 2.13 & \multicolumn{1}{r|}{0.40} & 0.15 & \multicolumn{1}{r|}{0.03} & 0.79 & 0.73 \\ \hline
\multicolumn{1}{l|}{GPT-2-PNV} & 2.15 & \multicolumn{1}{r|}{0.41} & 0.16 & \multicolumn{1}{r|}{0.08} & 0.95 & 0.94 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 2.17 & \multicolumn{1}{r|}{0.40} & 0.17 & \multicolumn{1}{r|}{0.08} & 0.98 & 0.91 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ F}} & \textbf{2.08} & \multicolumn{1}{r|}{\textbf{0.42}} & \textbf{0.17} & \multicolumn{1}{r|}{\textbf{0.09}} & \textbf{0.96} & \textbf{0.95} \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 2.22 & \multicolumn{1}{r|}{0.40} & 0.15 & \multicolumn{1}{r|}{0.09} & 0.98 & 0.92 \\ \hline
\multicolumn{1}{l|}{LLAMA-NV} & 3.09 & \multicolumn{1}{r|}{0.29} & 0.05 & \multicolumn{1}{r|}{0.03} & 0.83 & 0.66 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 3.13 & \multicolumn{1}{r|}{0.28} & 0.05 & \multicolumn{1}{r|}{0.04} & 0.71 & 0.70 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ F}} & \textbf{3.01} & \multicolumn{1}{r|}{\textbf{0.27}} & \textbf{0.05} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.87} & \textbf{0.66} \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 2.99 & \multicolumn{1}{r|}{0.27} & 0.06 & \multicolumn{1}{r|}{0.03} & 0.78 & 0.64 \\ \hhline{=======}
\multicolumn{7}{c}{\textbf{Stage 3 (Validation)}} \\ \hline
\multicolumn{1}{l|}{Flan-T5-P} & 2.26 & \multicolumn{1}{r|}{0.36} & 0.11 & \multicolumn{1}{r|}{0.028} & 0.80 & 0.78 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 2.22 & \multicolumn{1}{r|}{0.37} & 0.11 & \multicolumn{1}{r|}{0.04} & 0.85 & 0.78 \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 2.25 & \multicolumn{1}{r|}{0.38} & 0.10 & \multicolumn{1}{r|}{0.02} & 0.85 & 0.78 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ EF}} & \textbf{2.19} & \multicolumn{1}{r|}{\textbf{0.40}} & \textbf{0.12} & \multicolumn{1}{r|}{\textbf{0.02}} & \textbf{0.85} & \textbf{0.78} \\ \hline
\multicolumn{1}{l|}{GPT-2-PNV} & 1.97 & \multicolumn{1}{r|}{0.45} & 0.20 & \multicolumn{1}{r|}{0.07} & 0.92 & 0.93 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ E}} & \textbf{2.02} & \multicolumn{1}{r|}{\textbf{0.43}} & \textbf{0.20} & \multicolumn{1}{r|}{\textbf{0.07}} & \textbf{0.98} & \textbf{0.92} \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 1.98 & \multicolumn{1}{r|}{0.45} & 0.19 & \multicolumn{1}{r|}{0.08} & 0.95 & 0.93 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 2.05 & \multicolumn{1}{r|}{0.43} & 0.19 & \multicolumn{1}{r|}{0.08} & 0.99 & 0.93 \\ \hline
\multicolumn{1}{l|}{LLAMA-NV} & 3.15 & \multicolumn{1}{r|}{0.26} & 0.07 & \multicolumn{1}{r|}{0.03} & 0.67 & 0.74 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 3.17 & \multicolumn{1}{r|}{0.26} & 0.05 & \multicolumn{1}{r|}{0.03} & 0.80 & 0.71 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ F}} & \textbf{3.07} & \multicolumn{1}{r|}{\textbf{0.27}} & \textbf{0.08} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.75} & \textbf{0.79} \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.23 & \multicolumn{1}{r|}{0.25} & 0.05 & \multicolumn{1}{r|}{0.03} & 0.72 & 0.72
\end{tabular}}

==> tables/experiments/continuous_learning_extended.tex <==
\resizebox*{\linewidth}{!}{\begin{tabular}{lllllllllllllllllll}
\multicolumn{1}{c}{\textbf{Configuration}} & \multicolumn{6}{c}{\textbf{Stage1}} & \multicolumn{6}{c}{\textbf{Stage 2}} & \multicolumn{6}{c}{\textbf{Stage 3}} \\ \hline
\multicolumn{1}{c}{\textbf{}} & \multicolumn{2}{c}{\textbf{Performance}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{2}{c|}{\textbf{Task Completion}} & \multicolumn{2}{c}{\textbf{Performance}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{2}{c|}{\textbf{Task Completion}} & \multicolumn{2}{c}{\textbf{Performance}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{2}{c}{\textbf{Task Completion}} \\ \cline{2-19} 
\multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{PPL}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{Toxicity}} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c|}{\textbf{Success}} & \multicolumn{1}{c}{\textbf{PPL}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{Toxicity}} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c|}{\textbf{Success}} & \multicolumn{1}{c}{\textbf{PPL}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c}{\textbf{Toxicity}} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c}{\textbf{Success}} \\ \hline
\multicolumn{1}{l|}{\textbf{Flan-T5}} & 4.04 & \multicolumn{1}{l|}{0.45} & 0.20 & \multicolumn{1}{l|}{0.04} & 0.85 & \multicolumn{1}{l|}{0.84} & \textbf{4.13} & \multicolumn{1}{l|}{\textbf{0.45}} & \textbf{0.22} & \multicolumn{1}{l|}{\textbf{0.03}} & \textbf{0.83} & \multicolumn{1}{l|}{\textbf{0.84}} & 4.21 & \multicolumn{1}{l|}{0.41} & 0.19 & \multicolumn{1}{l|}{0.03} & 0.66 & 0.65 \\
\multicolumn{1}{l|}{+ Error Utterance} & \textbf{1.76} & \multicolumn{1}{l|}{\textbf{0.47}} & \textbf{0.24} & \multicolumn{1}{l|}{\textbf{0.03}} & \textbf{0.86} & \multicolumn{1}{l|}{\textbf{0.84}} & 4.18 & \multicolumn{1}{l|}{0.44} & 0.22 & \multicolumn{1}{l|}{0.03} & 0.80 & \multicolumn{1}{l|}{0.84} & 4.39 & \multicolumn{1}{l|}{0.41} & 0.19 & \multicolumn{1}{l|}{0.04} & 0.66 & 0.65 \\
\multicolumn{1}{l|}{+ User Reaction} & 1.80 & \multicolumn{1}{l|}{0.47} & 0.23 & \multicolumn{1}{l|}{0.03} & 0.81 & \multicolumn{1}{l|}{0.83} & 4.42 & \multicolumn{1}{l|}{0.45} & 0.23 & \multicolumn{1}{l|}{0.04} & 0.75 & \multicolumn{1}{l|}{0.83} & 4.32 & \multicolumn{1}{l|}{0.43} & 0.24 & \multicolumn{1}{l|}{0.02} & 0.70 & 0.82 \\
\multicolumn{1}{l|}{- Error Utterance} & 4.02 & \multicolumn{1}{l|}{0.46} & 0.22 & \multicolumn{1}{l|}{0.02} & 0.80 & \multicolumn{1}{l|}{0.83} & 3.95 & \multicolumn{1}{l|}{0.44} & 0.22 & \multicolumn{1}{l|}{0.02} & 0.74 & \multicolumn{1}{l|}{0.82} & \textbf{4.09} & \multicolumn{1}{l|}{\textbf{0.43}} & \textbf{0.23} & \multicolumn{1}{l|}{\textbf{0.02}} & \textbf{0.75} & \textbf{0.82} \\ \hline
\multicolumn{1}{l|}{\textbf{GPT-2}} & 3.31 & \multicolumn{1}{l|}{0.33} & 0.10 & \multicolumn{1}{l|}{0.08} & 0.77 & \multicolumn{1}{l|}{0.67} & 3.08 & \multicolumn{1}{l|}{0.30} & 0.11 & \multicolumn{1}{l|}{0.10} & 0.69 & \multicolumn{1}{l|}{0.74} & 3.19 & \multicolumn{1}{l|}{0.31} & 0.11 & \multicolumn{1}{l|}{0.07} & 0.76 & 0.79 \\
\multicolumn{1}{l|}{+ Error Utterance} & 3.13 & \multicolumn{1}{l|}{0.25} & 0.11 & \multicolumn{1}{l|}{0.08} & 0.80 & \multicolumn{1}{l|}{0.81} & 3.07 & \multicolumn{1}{l|}{0.24} & 0.09 & \multicolumn{1}{l|}{0.07} & 0.84 & \multicolumn{1}{l|}{0.78} & \textbf{2.86} & \multicolumn{1}{l|}{\textbf{0.27}} & \textbf{0.11} & \multicolumn{1}{l|}{\textbf{0.06}} & \textbf{0.84} & \textbf{0.80} \\
\multicolumn{1}{l|}{+ User Reaction} & \textbf{3.27} & \multicolumn{1}{l|}{\textbf{0.22}} & \textbf{0.10} & \multicolumn{1}{l|}{\textbf{0.09}} & \textbf{0.85} & \multicolumn{1}{l|}{\textbf{0.81}} & 3.18 & \multicolumn{1}{l|}{0.23} & 0.09 & \multicolumn{1}{l|}{0.09} & 0.82 & \multicolumn{1}{l|}{0.81} & 3.31 & \multicolumn{1}{l|}{0.27} & 0.11 & \multicolumn{1}{l|}{0.08} & 0.84 & 0.80 \\
\multicolumn{1}{l|}{- Error Utterance} & 3.03 & \multicolumn{1}{l|}{0.23} & 0.09 & \multicolumn{1}{l|}{0.10} & 0.78 & \multicolumn{1}{l|}{0.80} & \textbf{3.07} & \multicolumn{1}{l|}{\textbf{0.24}} & \textbf{0.11} & \multicolumn{1}{l|}{\textbf{0.09}} & \textbf{0.84} & \multicolumn{1}{l|}{\textbf{0.80}} & 2.86 & \multicolumn{1}{l|}{0.27} & 0.11 & \multicolumn{1}{l|}{0.08} & 0.83 & 0.79 \\ \hline
\multicolumn{1}{l|}{\textbf{LLAMA}} & \textbf{3.19} & \multicolumn{1}{l|}{\textbf{0.29}} & \textbf{0.05} & \multicolumn{1}{l|}{\textbf{0.03}} & \textbf{0.83} & \multicolumn{1}{l|}{\textbf{0.66}} & 3.33 & \multicolumn{1}{l|}{0.24} & 0.07 & \multicolumn{1}{l|}{0.03} & 0.75 & \multicolumn{1}{l|}{0.65} & \textbf{3.13} & \multicolumn{1}{l|}{\textbf{0.29}} & \textbf{0.05} & \multicolumn{1}{l|}{\textbf{0.03}} & \textbf{0.83} & \textbf{0.66} \\
\multicolumn{1}{l|}{+ Error Utterance} & 3.57 & \multicolumn{1}{l|}{0.22} & 0.05 & \multicolumn{1}{l|}{0.03} & 0.74 & \multicolumn{1}{l|}{0.49} & 3.53 & \multicolumn{1}{l|}{0.22} & 0.03 & \multicolumn{1}{l|}{0.04} & 0.69 & \multicolumn{1}{l|}{0.59} & 3.26 & \multicolumn{1}{l|}{0.26} & 0.08 & \multicolumn{1}{l|}{0.03} & 0.75 & 0.77 \\
\multicolumn{1}{l|}{+ User Reaction} & 3.31 & \multicolumn{1}{l|}{0.24} & 0.05 & \multicolumn{1}{l|}{0.03} & 0.66 & \multicolumn{1}{l|}{0.61} & 3.28 & \multicolumn{1}{l|}{0.25} & 0.04 & \multicolumn{1}{l|}{0.03} & 0.79 & \multicolumn{1}{l|}{0.67} & 3.25 & \multicolumn{1}{l|}{0.25} & 0.05 & \multicolumn{1}{l|}{0.03} & 0.72 & 0.72 \\
\multicolumn{1}{l|}{- Error Utterance} & 3.25 & \multicolumn{1}{l|}{0.27} & 0.05 & \multicolumn{1}{l|}{0.04} & 0.87 & \multicolumn{1}{l|}{0.66} & \textbf{3.30} & \multicolumn{1}{l|}{\textbf{0.27}} & \textbf{0.05} & \multicolumn{1}{l|}{\textbf{0.03}} & \textbf{0.87} & \multicolumn{1}{l|}{\textbf{0.66}} & 3.15 & \multicolumn{1}{l|}{0.28} & 0.08 & \multicolumn{1}{l|}{0.03} & 0.68 & 0.78
\end{tabular}}

==> tables/experiments/continuous_learning_test.tex <==
\resizebox*{0.9\linewidth}{!}{\begin{tabular}{lrrrrrr}
\multicolumn{1}{c}{\textbf{Experiment}} & \multicolumn{2}{c}{\textbf{Performance}} & \multicolumn{2}{c}{\textbf{Text Quality}} & \multicolumn{2}{c}{\textbf{Task Completion}} \\ \hline
\multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{PPL}} & \multicolumn{1}{c|}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{Toxicity}} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c}{\textbf{Success}} \\ \hhline{=======}
\multicolumn{7}{c}{\textbf{Stage 1 (Test)}} \\ \hline
\multicolumn{1}{l|}{Flan-T5-P} & 4.04 & \multicolumn{1}{r|}{0.45} & 0.20 & \multicolumn{1}{r|}{0.04} & 0.85 & 0.84 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ E}} & \textbf{1.76} & \multicolumn{1}{r|}{\textbf{0.47}} & \textbf{0.24} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.86} & \textbf{0.84} \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 4.02 & \multicolumn{1}{r|}{0.46} & 0.22 & \multicolumn{1}{r|}{0.02} & 0.80 & 0.83 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 4.24 & \multicolumn{1}{r|}{0.47} & 0.23 & \multicolumn{1}{r|}{0.03} & 0.81 & 0.83 \\ \hline
\multicolumn{1}{l|}{GPT-2-PNV} & 3.31 & \multicolumn{1}{r|}{0.33} & 0.10 & \multicolumn{1}{r|}{0.08} & 0.77 & 0.67 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ E}} & \textbf{3.13} & \multicolumn{1}{r|}{\textbf{0.25}} & \textbf{0.11} & \multicolumn{1}{r|}{\textbf{0.08}} & \textbf{0.80} & \textbf{0.81} \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 3.03 & \multicolumn{1}{r|}{0.23} & 0.09 & \multicolumn{1}{r|}{0.09} & 0.78 & 0.80 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.27 & \multicolumn{1}{r|}{0.22} & 0.10 & \multicolumn{1}{r|}{0.09} & 0.85 & 0.81 \\ \hline
\multicolumn{1}{l|}{LLAMA-NV} & 3.19 & \multicolumn{1}{r|}{0.29} & 0.05 & \multicolumn{1}{r|}{0.03} & 0.83 & 0.66 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 3.57 & \multicolumn{1}{r|}{0.22} & 0.05 & \multicolumn{1}{r|}{0.03} & 0.74 & 0.49 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ F}} & \textbf{3.25} & \multicolumn{1}{r|}{\textbf{0.27}} & \textbf{0.05} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.87} & \textbf{0.66} \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.31 & \multicolumn{1}{r|}{0.24} & 0.05 & \multicolumn{1}{r|}{0.03} & 0.66 & 0.61 \\ \hhline{=======}
\multicolumn{7}{c}{\textbf{Stage 2 (Test)}} \\ \hline
\multicolumn{1}{l|}{\textbf{Flan-T5-P}} & \textbf{4.13} & \multicolumn{1}{r|}{\textbf{0.45}} & \textbf{0.22} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.83} & \textbf{0.84} \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 4.18 & \multicolumn{1}{r|}{0.44} & 0.22 & \multicolumn{1}{r|}{0.03} & 0.80 & 0.84 \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 3.95 & \multicolumn{1}{r|}{0.44} & 0.22 & \multicolumn{1}{r|}{0.02} & 0.74 & 0.82 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 4.42 & \multicolumn{1}{r|}{0.45} & 0.23 & \multicolumn{1}{r|}{0.03} & 0.75 & 0.83 \\ \hline
\multicolumn{1}{l|}{GPT-2-PNV} & 3.08 & \multicolumn{1}{r|}{0.30} & 0.11 & \multicolumn{1}{r|}{0.10} & 0.69 & 0.74 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 3.07 & \multicolumn{1}{r|}{0.24} & 0.09 & \multicolumn{1}{r|}{0.07} & 0.84 & 0.78 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ F}} & \textbf{2.95} & \multicolumn{1}{r|}{\textbf{0.27}} & \textbf{0.11} & \multicolumn{1}{r|}{\textbf{0.09}} & \textbf{0.84} & \textbf{0.80} \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.18 & \multicolumn{1}{r|}{0.23} & 0.09 & \multicolumn{1}{r|}{0.09} & 0.82 & 0.81 \\ \hline
\multicolumn{1}{l|}{LLAMA-NV} & 3.33 & \multicolumn{1}{r|}{0.24} & 0.07 & \multicolumn{1}{r|}{0.03} & 0.75 & 0.65 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 3.53 & \multicolumn{1}{r|}{0.22} & 0.03 & \multicolumn{1}{r|}{0.04} & 0.69 & 0.59 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ F}} & \textbf{3.30} & \multicolumn{1}{r|}{\textbf{0.27}} & \textbf{0.05} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.87} & \textbf{0.66} \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.28 & \multicolumn{1}{r|}{0.25} & 0.04 & \multicolumn{1}{r|}{0.03} & 0.79 & 0.67 \\ \hhline{=======}
\multicolumn{7}{c}{\textbf{Stage 3 (Test)}} \\ \hline
\multicolumn{1}{l|}{Flan-T5-P} & 4.21 & \multicolumn{1}{r|}{0.41} & 0.19 & \multicolumn{1}{r|}{0.03} & 0.66 & 0.65 \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 4.39 & \multicolumn{1}{r|}{0.41} & 0.19 & \multicolumn{1}{r|}{0.04} & 0.66 & 0.65 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ F}} & \textbf{4.09} & \multicolumn{1}{r|}{\textbf{0.43}} & \textbf{0.23} & \multicolumn{1}{r|}{\textbf{0.02}} & \textbf{0.75} & \textbf{0.82} \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 4.32 & \multicolumn{1}{r|}{0.43} & 0.24 & \multicolumn{1}{r|}{0.01} & 0.70 & 0.82 \\ \hline
\multicolumn{1}{l|}{GPT-2-PNV} & 3.19 & \multicolumn{1}{r|}{0.31} & 0.11 & \multicolumn{1}{r|}{0.07} & 0.76 & 0.79 \\ \hline
\multicolumn{1}{l|}{\textbf{\quad+ E}} & \textbf{2.86} & \multicolumn{1}{r|}{\textbf{0.27}} & \textbf{0.11} & \multicolumn{1}{r|}{\textbf{0.06}} & \textbf{0.84} & \textbf{0.80} \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 3.29 & \multicolumn{1}{r|}{0.28} & 0.11 & \multicolumn{1}{r|}{0.08} & 0.83 & 0.79 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.31 & \multicolumn{1}{r|}{0.27} & 0.11 & \multicolumn{1}{r|}{0.08} & 0.84 & 0.80 \\ \hline
\multicolumn{1}{l|}{\textbf{LLAMA-NV}} & \textbf{3.13} & \multicolumn{1}{r|}{\textbf{0.29}} & \textbf{0.05} & \multicolumn{1}{r|}{\textbf{0.03}} & \textbf{0.83} & \textbf{0.66} \\ \hline
\multicolumn{1}{l|}{\quad+ E} & 3.26 & \multicolumn{1}{r|}{0.26} & 0.08 & \multicolumn{1}{r|}{0.03} & 0.75 & 0.77 \\ \hline
\multicolumn{1}{l|}{\quad+ F} & 3.25 & \multicolumn{1}{r|}{0.28} & 0.08 & \multicolumn{1}{r|}{0.03} & 0.68 & 0.78 \\ \hline
\multicolumn{1}{l|}{\quad+ EF} & 3.25 & \multicolumn{1}{r|}{0.25} & 0.05 & \multicolumn{1}{r|}{0.03} & 0.72 & 0.72
\end{tabular}}

==> tables/experiments/error_experiments.tex <==
\resizebox*{\linewidth}{!}{\begin{tabular}{lrrrrrrrrr}
\multicolumn{1}{c}{\textbf{Experiment}} & \multicolumn{3}{c}{\textbf{Performance}} & \multicolumn{4}{c}{\textbf{Task Completion}} & \multicolumn{2}{c}{\textbf{Quality}} \\ \hline
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{BertScore}} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c}{\textbf{Success}} & \multicolumn{1}{c}{\textbf{Intent Acc}} & \multicolumn{1}{c|}{\textbf{Slot Acc}} & \textbf{Toxicity} & \textbf{Q²} \\ \hline
\multicolumn{1}{l|}{FLAN-T5 +E} & 42.4 (\textcolor{negative_color}{\textbf{--4.3}}) & 19.3 (\textcolor{negative_color}{\textbf{--1.7}}) & \multicolumn{1}{l|}{87.8 (\textcolor{negative_color}{\textbf{--1.1}})} & 92.6 (\textcolor{positive_color}{\textbf{+8.7}}) & 90.2 (\textcolor{positive_color}{\textbf{+7.0}}) & 75.3 (\textcolor{positive_color}{\textbf{+14.1}}) & \multicolumn{1}{l|}{76.2 (\textcolor{positive_color}{\textbf{+17.9}})} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +ET} & 41.4 (\textcolor{negative_color}{\textbf{--5.3}}) & 19.8 (\textcolor{negative_color}{\textbf{--1.2}}) & \multicolumn{1}{l|}{87.8 (\textcolor{negative_color}{\textbf{--1.1}})} & 96.8 (\textcolor{positive_color}{\textbf{+12.9}}) & 92.7 (\textcolor{positive_color}{\textbf{+9.5}}) & 72.5 (\textcolor{positive_color}{\textbf{+11.3}}) & \multicolumn{1}{l|}{76.7 (\textcolor{positive_color}{\textbf{+18.4}})} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +F} & 41.3 (\textcolor{negative_color}{\textbf{--5.4}}) & 19.3 (\textcolor{negative_color}{\textbf{--1.7}}) & \multicolumn{1}{l|}{87.6 (\textcolor{negative_color}{\textbf{--1.3}})} & 96.6 (\textcolor{positive_color}{\textbf{+12.7}}) & 94.1 (\textcolor{positive_color}{\textbf{+10.9}}) & 69.0 (\textcolor{positive_color}{\textbf{+7.8}}) & \multicolumn{1}{l|}{76.2 (\textcolor{positive_color}{\textcolor{positive_color}{\textbf{+17.9}}})} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +ET +F} & 43.4 (\textcolor{negative_color}{\textbf{--3.3}}) & 22.1 (\textcolor{positive_color}{\textbf{+1.1}}) & \multicolumn{1}{l|}{88.2 (\textcolor{negative_color}{--0.7})} & 96.9 (\textcolor{positive_color}{\textbf{+13.0}}) & 95.3 (\textcolor{positive_color}{\textbf{+12.1}}) & 83.5 (\textcolor{positive_color}{\textbf{+22.3}}) & \multicolumn{1}{l|}{77.2 (\textcolor{positive_color}{\textbf{+18.9}})} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{GPT-2 +E} & 31.5 (\textcolor{negative_color}{\textbf{--3.6}}) & 8.4 (\textcolor{negative_color}{\textbf{--2.0}}) & \multicolumn{1}{l|}{86.5 (\textcolor{negative_color}{--0.6})} & 93.6  (\textcolor{positive_color}{\textbf{+9.5}}) & 89.7 (\textcolor{positive_color}{\textbf{+5.9}}) & 84.0 (\textcolor{positive_color}{\textbf{+8.6}}) & \multicolumn{1}{l|}{80.8 (\textcolor{positive_color}{\textbf{+13.5}})} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +ET} & 29.2 (\textcolor{negative_color}{\textbf{--5.9}}) & 8.0 (\textcolor{negative_color}{\textbf{--2.4}}) & \multicolumn{1}{l|}{86.2 (\textcolor{negative_color}{--0.9})} & 92.4 (\textcolor{positive_color}{\textbf{+8.3}}) & 91.7 (\textcolor{positive_color}{\textbf{+7.9}}) & 84.3 (\textcolor{positive_color}{\textbf{+8.9}}) & \multicolumn{1}{l|}{79.3 (\textcolor{positive_color}{\textbf{+12.0}})} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +F} & 30.0 (\textcolor{negative_color}{\textbf{--5.1}}) & 8.3 (\textcolor{negative_color}{\textbf{--2.1}}) & \multicolumn{1}{l|}{86.3 (\textcolor{negative_color}{--0.8})} & 98.9 (\textcolor{positive_color}{\textbf{+14.8}}) & 96.5 (\textcolor{positive_color}{\textbf{+12.7}}) & 83.0 (\textcolor{positive_color}{\textbf{+7.6}}) & \multicolumn{1}{l|}{80.3 (\textcolor{positive_color}{\textbf{+13.0}})} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +ET +F} & 30.3 (\textcolor{negative_color}{\textbf{--4.8}}) & 9.7 (\textcolor{negative_color}{--0.7}) & \multicolumn{1}{l|}{86.4 (\textcolor{negative_color}{--0.7})} & 94.7 (\textcolor{positive_color}{\textbf{+10.6}}) & 93.3 (\textcolor{positive_color}{\textbf{+9.5}}) & 88.0 (\textcolor{positive_color}{\textbf{+12.6}}) & \multicolumn{1}{l|}{80.8 (\textcolor{positive_color}{\textbf{+13.5}})} & 0.01 &  \\ \hline
\multicolumn{1}{l|}{LLaMA + E} & \multicolumn{1}{r}{30.6} & \multicolumn{1}{r}{10.2} & \multicolumn{1}{r|}{83.9} & \multicolumn{1}{r}{98.8} & \multicolumn{1}{r}{94.3} & \multicolumn{1}{r}{81.0} & \multicolumn{1}{r|}{75.4} & 0.03 &  \\ \hline
\multicolumn{1}{l|}{\quad +ET} & \multicolumn{1}{r}{31.7} & 12.2 & \multicolumn{1}{r|}{87.4} & \multicolumn{1}{r}{96.4} & \multicolumn{1}{r}{91.2} & \multicolumn{1}{r}{83.8} & \multicolumn{1}{r|}{76.6} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +F} & \multicolumn{1}{r}{29.6} & 9.2 & \multicolumn{1}{r|}{86.0} & \multicolumn{1}{r}{96.2} & \multicolumn{1}{r}{98.7} & \multicolumn{1}{r}{82.8} & \multicolumn{1}{r|}{76.7} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +ET +F} & \multicolumn{1}{r}{27.9} & 7.7 & \multicolumn{1}{r|}{85.4} & \multicolumn{1}{r}{97.6} & \multicolumn{1}{r}{95.2} & \multicolumn{1}{r}{83.0} & \multicolumn{1}{r|}{73.8} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{LLaMA-2 +E} & \multicolumn{1}{r}{23.5} & 5.3 & \multicolumn{1}{r|}{82.7} & \multicolumn{1}{r}{92.1} & \multicolumn{1}{r}{95.2} & \multicolumn{1}{r}{63.5} & \multicolumn{1}{r|}{70.1} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +ET} & \multicolumn{1}{r}{24.1} & \multicolumn{1}{r}{7.9} & \multicolumn{1}{r|}{77.4} & \multicolumn{1}{r}{93.1} & \multicolumn{1}{r}{95.7} & \multicolumn{1}{r}{46.3} & \multicolumn{1}{r|}{47.2} & 0.01 &  \\ \hline
\multicolumn{1}{l|}{\quad +F} & \multicolumn{1}{r}{24.5} & \multicolumn{1}{r}{6.9} & \multicolumn{1}{r|}{78.8} & \multicolumn{1}{r}{94.9} & \multicolumn{1}{r}{93.2} & \multicolumn{1}{r}{47.8} & \multicolumn{1}{r|}{49.8} & 0.02 &  \\ \hline
\multicolumn{1}{l|}{\quad +ET +F} & \multicolumn{1}{r}{25.0} & \multicolumn{1}{r}{9.2} & \multicolumn{1}{r|}{80.1} & \multicolumn{1}{r}{67.8} & \multicolumn{1}{r}{69.8} & \multicolumn{1}{r}{33.8} & \multicolumn{1}{r|}{33.8} & 0.03 & 
\end{tabular}}

==> tables/experiments/tod_qa_comparison.tex <==
\resizebox*{\linewidth}{!}{
\begin{tabular}{lllrrr}
 &  &  & \multicolumn{1}{l}{\textbf{F1}} & \multicolumn{1}{l}{\textbf{BLEU}} & \multicolumn{1}{l}{\textbf{BertScore}} \\ \hline
\multicolumn{1}{l|}{\multirow{10}{*}{FLAN-T5}} & \multicolumn{1}{l|}{\multirow{5}{*}{QA}} & \multicolumn{1}{l|}{FLAN-T5} & 47.6 & 25.9 & 88.1 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Emotions} & 53.5 & 31.3 & 89.7 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Demographics} & 52.2 & 30.2 & 88.9 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Demographics\end{tabular}} & 50.0 & 28.2 & 88.7 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Generation Error\\ + User Reaction\end{tabular}} & 48.8 & 32.0 & 89.2 \\ \cline{2-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\multirow{5}{*}{ToD}} & \multicolumn{1}{l|}{FLAN-T5} & 33.6 & 5.2 & 87.2 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Emotions} & 36.7 & 6.8 & 88.4 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Demographics} & 32.9 & 5.6 & 86.5 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Demographics\end{tabular}} & 32.3 & 5.8 & 87.6 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Generation Error\\ + User Reaction\end{tabular}} & 30.9 & 5.4 & 85.5 \\ \hline
\multicolumn{1}{l|}{\multirow{10}{*}{GPT-2}} & \multicolumn{1}{l|}{\multirow{5}{*}{QA}} & \multicolumn{1}{l|}{GPT-2} & 37.4 & 12.1 & 89.0 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Emotions} & 40.6 & 16.2 & 89.6 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Demographics} & 38.6 & 10.1 & 89.6 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Demographics\end{tabular}} & 40.9 & 11.2 & 89.2 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Demographics\\ + Generation Error\\ + User Reaction\end{tabular}} & 35.3 & 11.3 & 86.4 \\ \cline{2-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\multirow{5}{*}{ToD}} & \multicolumn{1}{l|}{GPT-2} & 34.4 & 11.1 & 86.3 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Emotions} & 34.1 & 10.7 & 86.1 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Demographics} & 31.7 & 9.8 & 85.9 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Demographics\end{tabular}} & 34.5 & 11.6 & 86.4 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Demographics\\ + Generation Error\\ + User Reaction\end{tabular}} & 26.2 & 17.9 & 85.6 \\ \hline
\multicolumn{1}{l|}{\multirow{10}{*}{Llama 2}} & \multicolumn{1}{l|}{\multirow{5}{*}{QA}} & \multicolumn{1}{l|}{Llama 2} & 34.0 & 12.7 & 84.8 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Emotions} & 32.1 & 10.6 & 84.9 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Demographics} & 31.5 & 6.2 & 86.1 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Demographics\end{tabular}} & 29.1 & 6.1 & 85.9 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + User Reaction\end{tabular}} & 24.4 & 7.9 & 76.0 \\ \cline{2-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\multirow{5}{*}{ToD}} & \multicolumn{1}{l|}{Llama 2} & 26.5 & 8.0 & 86.6 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Emotions} & 28.3 & 5.9 & 85.4 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{+ Demographics} & 28.9 & 5.6 & 85.7 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + Demographics\end{tabular}} & 26.5 & 8.0 & 86.6 \\ \cline{3-6} 
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}+ Emotions\\ + User Reaction\end{tabular}} & 22.9 & 4.7 & 87.4
\end{tabular}}

==> tables/experiments/validation_data.tex <==
\resizebox*{\linewidth}{!}{\begin{tabular}{llrrrrrrrrr}
\multicolumn{1}{c}{\textbf{}} &  \multicolumn{1}{c}{\textbf{Experiment}} & \multicolumn{4}{c}{\textbf{Task Completion}} & \multicolumn{2}{c}{\textbf{Quality}} & \multicolumn{3}{c}{\textbf{Generation Accuracy}} \\ \hline
 & \multicolumn{1}{l}{} & \multicolumn{1}{c}{\textbf{Inform}} & \multicolumn{1}{c}{\textbf{Success}} & \multicolumn{1}{c}{\textbf{Intent Acc.}} & \multicolumn{1}{c|}{\textbf{Slot Acc.}} & \multicolumn{1}{c}{\textbf{Toxicity}} & \multicolumn{1}{c|}{\textbf{Q²}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{BLEU}} & \multicolumn{1}{c|}{\textbf{BertScore}} \\ \hhline{===========}
 
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Flan-T5 \\ Feedback-Free\end{tabular}} & \multicolumn{1}{l|}{Flan-T5} & 84.6 & 81.2 & 93.8 & \multicolumn{1}{r|}{64.0} & 0.02 & \multicolumn{1}{r|}{51.2} & 41.9 & 16.2 & 87.4\\ \hline

\multicolumn{1}{l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Feedback\end{tabular}}}  & \multicolumn{1}{l|}{\quad+Generation Error} & \multicolumn{1}{r}{89.2 \textsubscript{\textcolor{positive_color}{(+4.6)}}} & \multicolumn{1}{r}{84.1 \textsubscript{\textcolor{positive_color}{(+2.9)}}} & \multicolumn{1}{r}{95.0 \textsubscript{\textcolor{positive_color}{(+1.2)}}} & \multicolumn{1}{r|}{86.7 \textsubscript{\textcolor{positive_color}{(+22.7)}}} & 0.02& \multicolumn{1}{r|}{54.6 \textsubscript{\textcolor{positive_color}{(+3.4)}}} & \multicolumn{1}{r}{41.2 \textsubscript{\textcolor{negative_color}{(--0.7)}}} & \multicolumn{1}{r}{15.4 \textsubscript{\textcolor{negative_color}{(--0.8)}}} & 87.6 \textsubscript{\textcolor{positive_color}{(+0.2)}} \\ \cline{2-11}
\multicolumn{1}{c|}{}  & \multicolumn{1}{l|}{\quad+User Reaction} & \multicolumn{1}{r}{83.2 \textsubscript{\textcolor{negative_color}{(--1.2)}}} & \multicolumn{1}{r}{81.7 \textsubscript{\textcolor{positive_color}{(+0.5)}}} & \multicolumn{1}{r}{91.8 \textsubscript{\textcolor{negative_color}{(--2.0)}}} & \multicolumn{1}{r|}{87.0 \textsubscript{\textcolor{positive_color}{(+23.0)}}} & 0.02 & \multicolumn{1}{r|}{53.9 \textsubscript{\textcolor{positive_color}{(+2.7)}}} & \multicolumn{1}{r}{42.7 \textsubscript{\textcolor{positive_color}{(+0.8)}}} & \multicolumn{1}{r}{16.0 \textsubscript{\textcolor{negative_color}{(--0.2)}}} & 88.9 \textsubscript{\textcolor{positive_color}{(+2.5)}} \\ \cline{2-11}
\multicolumn{1}{c|}{}  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\quad+Generation Error\\     \quad+User Reaction\end{tabular}} & \multicolumn{1}{r}{89.5 \textsubscript{\textcolor{positive_color}{(+4.9)}}} & \multicolumn{1}{r}{86.2 \textsubscript{\textcolor{positive_color}{(+5.0)}}} & \multicolumn{1}{r}{97.0 \textsubscript{\textcolor{positive_color}{(+3.2)}}} & \multicolumn{1}{r|}{88.5 \textsubscript{\textcolor{positive_color}{(+24.5)}}} & 0.02 & \multicolumn{1}{r|}{58.2 \textsubscript{\textcolor{positive_color}{(+7.0)}}} & \multicolumn{1}{r}{42.9 \textsubscript{\textcolor{positive_color}{(+1.0)}}} & \multicolumn{1}{r}{16.3 \textsubscript{\textcolor{positive_color}{(+0.1)}}} & 87.8 \textsubscript{\textcolor{positive_color}{(+0.4)}} \\ \hhline{===========}

\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}GPT-2 \\ Feedback-Free\end{tabular}} & \multicolumn{1}{l|}{GPT-2} & 83.2 & 82.1 & 96.5 & \multicolumn{1}{r|}{93.3} & 0.02 & \multicolumn{1}{r|}{22.1} & 50.1 & 27.1 & 90.5 \\ \hline

\multicolumn{1}{l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Feedback\end{tabular}}} & \multicolumn{1}{l|}{\quad+Generation Error} &  \multicolumn{1}{r}{89.2 \textsubscript{\textcolor{positive_color}{(+6.0)}}} & \multicolumn{1}{r}{90.1 \textsubscript{\textcolor{positive_color}{(+8.0)}}} & \multicolumn{1}{r}{98.0 \textsubscript{\textcolor{positive_color}{(+1.5)}}} & \multicolumn{1}{r|}{92.9 \textsubscript{\textcolor{negative_color}{(--0.4)}}} & 0.02 & \multicolumn{1}{r|}{25.6 \textsubscript{\textcolor{positive_color}{(+3.5)}}} & \multicolumn{1}{r}{53.1 \textsubscript{\textcolor{positive_color}{(+3.0)}}} & \multicolumn{1}{r}{30.2 \textsubscript{\textcolor{positive_color}{(+3.1)}}} & \multicolumn{1}{r}{90.6 \textsubscript{\textcolor{positive_color}{(+0.1)}}} \\ \cline{2-11}
\multicolumn{1}{c|}{}  & \multicolumn{1}{l|}{\quad+User Reaction} & \multicolumn{1}{r}{88.5 \textsubscript{\textcolor{positive_color}{(+2.3)}}} & \multicolumn{1}{r}{86.1 \textsubscript{\textcolor{positive_color}{(+4.0)}}} & \multicolumn{1}{r}{94.6 \textsubscript{\textcolor{negative_color}{(--1.9)}}} & \multicolumn{1}{r|}{93.9 \textsubscript{\textcolor{positive_color}{(+0.6)}}} & 0.02 & \multicolumn{1}{r|}{29.4 \textsubscript{\textcolor{positive_color}{(+7.3)}}} & \multicolumn{1}{r}{50.8 \textsubscript{\textcolor{negative_color}{(--0.3)}}} & \multicolumn{1}{r}{26.8 \textsubscript{\textcolor{negative_color}{(--0.3)}}} & \multicolumn{1}{r}{89.8 \textsubscript{\textcolor{negative_color}{(--0.7)}}}\\ \cline{2-11}
\multicolumn{1}{c|}{}  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\quad+Generation Error\\     \quad+User Reaction\end{tabular}} &  \multicolumn{1}{r}{90.2 \textsubscript{\textcolor{positive_color}{(+7.0)}}} & \multicolumn{1}{r}{87.9 \textsubscript{\textcolor{positive_color}{(+5.8)}}} & \multicolumn{1}{r}{98.0 \textsubscript{\textcolor{positive_color}{(+1.5)}}} & \multicolumn{1}{r|}{94.9 \textsubscript{\textcolor{positive_color}{(+1.6)}}} & 0.02 & \multicolumn{1}{r|}{28.1 \textsubscript{\textcolor{positive_color}{(+6.0)}}} & \multicolumn{1}{r}{51.5 \textsubscript{\textcolor{positive_color}{(+1.4)}}} & \multicolumn{1}{r}{26.2 \textsubscript{\textcolor{negative_color}{(--0.9)}}} & \multicolumn{1}{r}{90.2 \textsubscript{\textcolor{negative_color}{(--0.3)}}} \\ \hhline{===========}

\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Llama 2 \\ Feedback-Free\end{tabular}} & \multicolumn{1}{l|}{Llama 2} & 80.1 & 84.5 & 52.3 & \multicolumn{1}{r|}{56.7} & 0.01 & \multicolumn{1}{r|}{35.1} & 31.6 & 7.5 & \multicolumn{1}{r}{87.1} \\ \hline

\multicolumn{1}{l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Feedback\end{tabular}}}  & \multicolumn{1}{l|}{\quad+Generation Error} &  87.6 \textsubscript{\textcolor{positive_color}{(+7.5)}} & 85.4 \textsubscript{\textcolor{positive_color}{(+0.9)}} & 59.3 \textsubscript{\textcolor{positive_color}{(+7.0)}} & \multicolumn{1}{r|}{61.2 \textsubscript{\textcolor{positive_color}{(+4.5)}}} & 0.01 & \multicolumn{1}{r|}{36.7 \textsubscript{\textcolor{positive_color}{(+1.6)}}} & 31.4 \textsubscript{\textcolor{negative_color}{(--0.2)}} & 8.3 \textsubscript{\textcolor{positive_color}{(+0.8)}} & \multicolumn{1}{r}{87.7 \textsubscript{\textcolor{positive_color}{(+0.6)}}} \\ \cline{2-11}
\multicolumn{1}{c|}{}  & \multicolumn{1}{l|}{\quad+User Reaction} & 86.9 \textsubscript{\textcolor{positive_color}{(+6.8)}} & 84.2 \textsubscript{\textcolor{negative_color}{(--0.3)}} & 60.1 \textsubscript{\textcolor{positive_color}{(+7.8)}} & \multicolumn{1}{r|}{62.4 \textsubscript{\textcolor{positive_color}{(+5.7)}}} & 0.02 \textsubscript{\textcolor{negative_color}{(--0.01)}} & \multicolumn{1}{r|}{35.9 \textsubscript{\textcolor{positive_color}{(+0.8)}}} & 32.2 \textsubscript{\textcolor{positive_color}{(+0.6)}} & 8.5 \textsubscript{\textcolor{positive_color}{(+1.0)}} & \multicolumn{1}{r}{84.6 \textsubscript{\textcolor{negative_color}{(--2.5)}}} \\ \cline{2-11}
\multicolumn{1}{c|}{}  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\quad+Generation Error\\     \quad+User Reaction\end{tabular}} & 83.5 \textsubscript{\textcolor{positive_color}{(+3.4)}} & 84.1 \textsubscript{\textcolor{negative_color}{(--0.4)}} & 60.7 \textsubscript{\textcolor{positive_color}{(+8.4)}} & \multicolumn{1}{r|}{59.6 \textsubscript{\textcolor{positive_color}{(+2.9)}}} & 0.02 \textsubscript{\textcolor{negative_color}{(--0.01)}} & \multicolumn{1}{r|}{36.2 \textsubscript{\textcolor{positive_color}{(+1.1)}}} & 32.5 \textsubscript{\textcolor{positive_color}{(+0.9)}} & 8.5 \textsubscript{\textcolor{positive_color}{(+1.0)}} & \multicolumn{1}{r}{84.1 \textsubscript{\textcolor{negative_color}{(+3.0)}}}
\end{tabular}}





